Walk, Not Wait: Faster Sampling Over Online Social Networks

In this paper, we introduce a novel, general purpose, technique for faster sampling of nodes over an online social network. Specifically, unlike traditional random walk which wait for the convergence of sampling distribution to a predetermined target distribution - a waiting process that incurs a high query cost - we develop WALK-ESTIMATE, which starts with a much shorter random walk, and then proactively estimate the sampling probability for the node taken before using acceptance-rejection sampling to adjust the sampling probability to the predetermined target distribution. We present a novel backward random walk technique which provides provably unbiased estimations for the sampling probability, and demonstrate the superiority of WALK-ESTIMATE over traditional random walks through theoretical analysis and extensive experiments over real world online social networks.

==> cycle.tex <==
\subsection{Expected Cost of the IDEAL-WALK in Odd Cycle}
\label{sec:cycle}
In this section, we first find the expected cost of getting one sample after a walk of a length $k$ using our IDEAL-AR-SAMPLER algorithm in odd cycle of length $l$. Next, we show that there an optimal $k$, where the expected cost of IDEAL-AR-SAMPLER algorithm is less than the expected cost of the classical random walk. 

\begin{lemma}
\label{lm:cost_AR}
Given an odd cycle of length $l$, expected cost of IDEAL-AR-SAMPLER algorithm $(c_{AR}(k))$ after a walk of length $k$, $k \leq l-1$, is
\begin{equation}
\label{cost_AR}
\begin{cases}  
\frac{k*2^k}{l*({k+1 \choose \frac{k-l+1}{2} } + \sum_{i=0}^{\frac{k-3l+1} {2l}} {k+1 \choose il+(\frac{k-l+1}{2}\mod l) }) }
  &\mbox{if } k \equiv 0 \\ 
\frac{k}{l*V_{{k-1}_{min}}} & \mbox{if } k \equiv 1. \end{cases} \pmod{2}
\end{equation}
\end{lemma}
\begin{proof}
Consider a random walk of length $k$ on an odd cycle of length $l$, where $s$ is the seed node, $T$ is the transition matrix, and $V_k$ be the landing probability vector at step $k$. 

Since in a cycle, each node $i$ is connected to nodes $(i \pm 1) \mod l$ and $V_1[i] = T_{si}$, $V_k$ can be driven by a recursive formula:
\begin{equation}
V_k[i] = (V_{k-1}[(i+1) \mod l]+V_{k-1}[(i-1) \mod l])* \frac{1}{2}
\end{equation}

In odd cycle, starting from the seed node, if length of walk $(k)$ is an odd number, after random walk of length $k$ the seed node is a node with minimum landing probability, but if $k$ is an even number the nodes next to the seed node are the nodes with minimum landing probability at step $k$. Thus $V_{k_{min}}$ is given by:

\begin{equation}
\label{equ:minProb_recursive}
\begin{cases} V_{k}[(s+1) \mod l]=V_{k}[(s-1) \mod l] &\mbox{if } k \equiv 0 \\ 
V_{k}[s] & \mbox{if } k \equiv 1. \end{cases} \pmod{2}
\end{equation}

Thus the expected acceptance of a sample after a walk of length $k$ is given by:
\begin{equation}
\label{equ:expectedAcceptance}
E[X] = \sum_{i=0}^{l-1} V_{k}[i]* \frac {V_{k_{min}}}{V_{k}[i]} = l*V_{k_{min}}
\end{equation}

In the proposed k-step walk algorithm, getting one sample follows the geometric distribution due to the fact that it would be the first occurrence of accepting a sample after $n$ number of independent trials, each with accepting probability $E[X]$ in Equation~\ref{equ:expectedAcceptance}. Thus the expected cost of our algorithm ($c_{AR}$) which is the expected cost of getting one sample after a walk of a length $k$ would be:
\begin{equation}
\label{equ:cost-AR}
c_{AR}(k) = \frac{k}{l*V_{k_{min}}}
\end{equation}

Clearly, if length of walk is less than the length of cycle (two times of the diameter), i.e., $(k \leq l-1)$, the minimum landing probability at step $k$, $V_{k_{min}}$, is zero; otherwise, it is given by:

\begin{equation}
\label{equ:minProb}
\begin{cases}  \frac{1}{2^k}*({k+1 \choose \frac{k-l+1}{2} } + \sum_{i=0}^{\frac{k-3l+1} {2l}} {k+1 \choose il+(\frac{k-l+1}{2}\mod l) })  &\mbox{if } k \equiv 0 \\ 
V_{{k-1}_{min}} & \mbox{if } k \equiv 1. \end{cases} \pmod{2}
\end{equation}
Thus, Equation~\ref{equ:cost-AR} with $V_{k_{min}}$ in Equation~\ref{equ:minProb} give us the expected cost of IDEAL-AR-SAMPLER algorithm in the lemma~\ref{lm:cost_AR}.
\end{proof}

Next we compare the expected cost of the IDEAL-AR-SAMPLER algorithm with the expected cost of the classic random walk.
\begin{lemma}
Given an odd cycle of length $l$, expected cost of IDEAL-AR-SAMPLER algorithm ($c_{AR}(k)$) with a walk of length $k = \frac {l^2}{3} - 1$ is less than the expected cost of classic random walk ($c_{RW}$).
\end{lemma}
\begin{proof}
In random walk, since the visited node after the mixing time would be accepted as a sample, we use the mixing time of an odd cycle as the expected cost of the classic random walk. The second largest eigenvalue of an odd cycle and its mixing time is $ \lambda = 2*cos(2\pi/n)$ and~\cite{Levin:2008} proves that the mixing time of an odd cycle is bounded as:
\begin{align*}
(1/\gamma *\log (\frac{1}{2\epsilon})) & \leq t_{mix}(\epsilon) < 1+ 1/\gamma* \log (\frac{1}{\epsilon \pi_{min}})\\
\Omega(l^2) & \leq t_{mix} \leq O(l^2 \log l)
\end{align*}
Where $\gamma$ is the spectral gap, i.e., $\gamma = 1- \lambda$. Thus, the expected query cost per sample achieved by the random walk would be: 
\begin{equation}
\Omega(l^2) \leq c_{RW} \leq O(l^2 \log l)
\end{equation}

In order show that our algorithm is better than the simple random walk, we should find optimal value of the $k$ that minimizes expected cost of the IDEAL-AR-SAMPLER in Equation~\ref{cost_AR} and $c_{RW}(k) < l^2 < c_{RW}$. 

There are two observations:
\begin{itemize}
\item Since the number of steps in simple random walk is atleast $l^2$, the optimal value of the $k$ should be less than $l^2$.
\item If $k<l^2$, $\sum_{i=0}^{\frac{k-3l+1} {2l}} {k+1 \choose il+(\frac{k-l+1}{2}~mod~l) } = 0$. 
\end{itemize} 

Thus, we should find optimal value of the $k < l^2$ that minimizes:
\begin{equation}
c_{AR}(k) = \frac{k*2^k}{l*{k+1 \choose \frac{k-l+1}{2} } }
\end{equation}

Using the formal definition of the derivative, the optimal k should satisfy:
\begin{align*}
& \frac {c_{AR}(k)-c_{AR}(k-2)}{2} = 0\\
& 4k*{k-1 \choose \frac{k-l-1}{2} } - (k-2)*{k+1 \choose \frac{k-l+1}{2} } = 0\\
& (k+1)^2 - l^2 - (k-2)(k+1) = 0\\
& k = \frac {l^2}{3} - 1
\end{align*}

Where for $l \geq 1$ and $k = \frac {l^2}{3} - 1$, $c_{AR}(k) < c_{RW}$.
\end{proof}



==> mh.tex <==
\subsubsection{Extension to Metropolis-Hastings}
Given an arbitrary distribution $\pi$, Metropolis-Hastings method modifies the transition probability matrix of a graph so that the random walk on this graph with the modified probability transition matrix converges to an arbitrary distribution $\pi$. In sampling, Metropolis-Hastings Random Walk (MHRW) used to get a uniform samples. Due to the fact that MHRW designs the MCMC process with uniform sampling distribution, our Walk Algorithm can be modified easily to be used on this MCMC process and produce uniform samples with the significantly smaller query cost. 

The Forward step of the walk algorithm runs $n$ walks of length $k$, where at every walk it selects a random neighbor $v$ of the node $u$ and move to node $v$ with probability $\min\{1,\frac{|N(u)|}{|N(v)|}\}$, where $N(u)$ is the set of neighbors of $u$. Otherwise, it would stay at $u$. See the transition matrix of MHRW from equation (\ref{MH-transition}).

Thus given a seed node $s$ and length of walk $k$, the extended version of our walk algorithm is as follows.
\begin{itemize}
\item Estimate landing probability of the visited nodes at step $k$ using the Forward-Backward algorithm based on equation~\ref{MH-transition} and 14.
\item After the walk of length $k$ accept the last node $u$ with probability $\frac{p_{k_{min}}}{p_k(u)}$, where $p_{k_{min}}$ is the minimum estimated landing probability at step $k$.
\end{itemize}

%In the walk algorithm, Equation 14 is used to estimate the landing probability by the backward process. However, in the extended version of our algorithm it should be modified to:
%\begin{equation}
%p^{\sim}_t(u) = \frac{\sum _{v \in N(u)}P(v,u)}{\sum _{v \in N(u')}P(u',v)}p_{t-1}(u')
%\end{equation}




%There are only few changes that need to be applied in our 


